Variational Bayesian Filtering with Subspace Information for Extreme Spatio-Temporal Matrix Completion

Missing data is a common problem in real-world sensor data collection. The performance of various approaches to impute data degrade rapidly in the extreme scenarios of low data sampling and noisy sampling, a case present in many real-world problems in the field of traffic sensing and environment monitoring, etc. However, jointly exploiting the spatiotemporal and periodic structure, which is generally not captured by classical matrix completion approaches, can improve the imputation performance of sensor data in such real-world conditions. We present a Bayesian approach towards spatiotemporal matrix completion wherein we estimate the underlying temporarily varying subspace using a Variational Bayesian technique. We jointly couple the low-rank matrix completion with the state space autoregressive framework along with a penalty function on the slowly varying subspace to model the temporal and periodic evolution in the data. A major advantage of our method is that a critical parameter like the rank of the model is automatically tuned using the automatic relevance determination (ARD) approach, unlike most matrix/tensor completion techniques. We also propose a robust version of the above formulation, which improves the performance of imputation in the presence of outliers. We evaluate the proposed Variational Bayesian Filtering with Subspace Information (VBFSI) method to impute matrices in real-world traffic and air pollution data. Simulation results demonstrate that the proposed method outperforms the recent state-of-the-art methods and provides a sufficiently accurate imputation for different sampling rates. In particular, we demonstrate that fusing the subspace evolution over days can improve the imputation performance with even 15% of the data sampling.

==> introduction3.tex <==


\section{Introduction}
\begin{itemize}
    \item EMC different than MC
    \item why its different and what makes this different than standard MC\\
    why special constraint 
    why do we need to know the structure of data more accurately and our dependence on knowing/awareness of the structure of the data. 
    \item Motivation for EMC not coming out

\end{itemize}
\textbf{more context about static sensors}

Copious amounts of sensors are deployed in major cities for sensing the spatio-temporal variation in various urban environment characteristics like air pollution, traffic speed, etc.  Hitherto, the most common way of sensing data across a city is to deploy many stationary sensors or monitors across the city. Ideally, these static monitors should have a dense spatial and temporal coverage. Deploying static sensors in such large numbers for spatio-temporal coverage is not only expensive but also challenging to maintain, and as a result, most cities, especially in the developing world, have a sparse network of sensor monitors \cite{vardoulakis2005spatial}.  One way to improve the spatio-temporal data coverage is to use drive-by sensing or moving sensors that sample various parts of a region at different time instances.  \cite{intro_drive1,hasenfratz2015deriving}. Since one sensor can be used to sample many locations at different timestamps, the actual number of moving sensors needed is just a fraction of the total number of static sensors needed to get the same spatial coverage.
\par 
\textbf{Link missing}
Data acquired from both static and moving sensors contains missing data due to sensor malfunction, irregularity in sensor measurements, etc.  Additionally, the drive-by sensing scheme uses relatively fewer sensors resulting in high data ``gaps" in both spatial and temporal dimensions \cite{intro_drive1}.\textbf{ This motivates the problem of extreme matrix completion, where the percentage of data sampled may be as low as $10\%$.  Hence, a natural question to ask is: how to fill the missing entries within a reasonable error range? In addition to the missing entries, sensor measurements can be contaminated with outliers emerging from the sensor malfunctioning, communication errors, or impulse noises.} The occurrence of outliers in the measurements can further degrade the performance of data imputation. However, unlike the missing entries, the location and the value of outliers are unknown, which makes the problem more challenging. Therefore, the other question to ask is: how to estimate the missing data while detecting the noisy outliers?  The answer to the above questions lies in exploiting the underlying structure available in the data. For instance, both the air pollution \cite{sampson2011pragmatic} and the traffic \cite{min2011real} data exhibit joint spatial and temporal correlation as well as temporal periodicity, thereby generating redundancy that can be potentially exploited by performing an intelligent spatio-temporal extrapolation.   \par
 
\subsection{ Extreme Spatio Temporal Matrix Completion}
Data collected from the sensors in transportation and environment, etc., have spatial variability and follows slowly varying pattern over time. One way to exploit this spatiotemporal correlation is to represent the data in the form of a matrix, where one axis denotes the spatial variability, and the other axis indicates the temporal evolution.  
We motivate the problem of spatio-temporal matrix completion as follows. For a given day $d$, the data is represented in the form of a matrix $\X \in \mathcal{R}^{n \times t}$  where  $n$ and  $t$ are the numbers of spatial locations and time slots, respectively. The elements in this matrix are missing due to the moving sensor paradigm or sensor malfunctioning. The data will be highly sparse in the case of moving sensor paradigm where the sampling percentage can be as low as 10\%. Our goal is to estimate the missing entries in the matrix $\X$. We motivate a low-rank robust subspace filtering approach for online matrix imputation, specifically for the extreme scenario of very sparse spatio-temporal sensing. \textbf{why motivate and no connection}

One way of imputation is to exploit the low-rank structure available in the data. The data $\X$ is low rank because of the spatial correlation in the locations and the temporal correlation in the time slots \cite{asif2016matrix}. Further, the data represented in the matrix $\X$ is a time-series data. Enforcing only the low-rank structure in the data does not take into account the temporal variation (generally slow variation) of the data in a given location \cite{compare1}. We incorporate a state space model to capture the temporal evolution in the data. 
Moreover, exploiting reliable prior subspace information can reduce the sample complexity of matrix completion and improve the imputation performance \cite{prove1}. We update the subspace on day $d$ using the prior subspace estimated of day $d-1$ to capture the periodicity in the data. Incorporating this prior subspace can improve the performance for an extreme case of sparsely sampled data. 


\subsection{Our contribution and Approach}
In this paper, we propose a Variational Bayesian Spatiotemporal matrix completion to estimate the data even in the presence of extreme matrix completion where the percentage of data sampled may be as low as $10\%$. We observe that even with a fraction of observed data, we can estimate the remaining measurements with reasonable accuracy. 
This work exploits the spatiotemporal and periodic pattern in the measurements for extreme matrix completion with reasonable accuracy.  Firstly, we enforce a low-rank structure to the spatiotemporal data. Secondly, we enforce the state-space model on the temporal embeddings to capture the temporal evolution in the data. Thirdly, we enforce the subspace estimate for $d$ day of the matrix to be close to previously learned subspace distribution for $d-1$ day using the Mahalanobis distance. Exploiting the prior subspace over days results in a considerable reduction of the number of measurements required to estimate the matrix \cite{prove1,prove2} thereby boosting the performance in case of a low sampling rate.


We use the Variational Bayes approach to update the parameters in an iterative fashion. In our work, the subspace distribution is chosen to allow automatic relevance determination (ARD), and unlike the matrix or tensor completion methods, the algorithm parameters such as rank, noise powers need not be specified or tuned. We compare the performance of the proposed algorithm with various state-of-the-art algorithms on many real-world traffic and air quality datasets. The result shows that modeling the subspace evolution leads to improvement in performance even when a small percentage of random measurements are available for the purpose of imputation. A likely impact of our method is that cities with a low sensing budget can perform random drive-by sampling of the urban environment, and the suggested matrix completion framework can provide a reasonably accurate imputation leading to better decision making. \par 

Our main contribution can be summarized as follows.
\begin{itemize}
	\item  We propose Variational Bayesian Filtering with Subspace Information (VBFSI), a novel matrix completion framework that simultaneously models the low rank nature of the data, temporal evolution through a state space model, and periodicity through subspace tracking. 
	\item We experimentally showed that incorporating the prior subspace over days can improve imputation performance for extreme spatio temporal matrix completion i.e. for low data sampling.
	% <not clear> \item We also illustrate our subspace can reduce the sample complexity, thereby motivating VBFSI for extreme matrix completion.
	\item Critical parameter, like the rank of the model, is automatically tuned using the automatic relevance determination (ARD) approach. 
	\item  We also propose a Robust version of the VBFSI algorithm for imputing the data in the presence of outliers. 
	\item We conduct comprehensive experiments on real-world spatio-temporal datasets that show the efficacy of the proposed method over other state-of-the-art imputation methods. 
	
\end{itemize} 


% This work exploits the spatio temporal and periodic pattern in the measurements to even impute  the 85\% of the missing data with resonable accuracy. We use three loss functions to model the structure of the data. First we enforce a low rank structure to the spatio temporal data as shown in Fig \ref{fig1}. Second we enforce the auto regressive model on the temporal embeddings $v_t$ to capture the temporal evolution in the data. Third we enforce the subspace estimate  $\mathbf{U}$of the matrix to be close to previously learned subspace distribution $\mathbf{\hat{U}}$ using the Mahalanobis distance. 
% Exploiting the prior subspace over days and result in considerable reduction of the number of measurements required to estimate the matrix \cite{prove1,prove2} thereby boosting the performance in case of low sampling rate .
% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=0.5\textwidth]{image/pic1.png}
% 	\centering
% 	\caption{ Low rank Matrix completion }
% 	\label{fig1}
% \end{figure}
% All the parameters of the model are learned in a iterative fashion using Variational Bayesian. Variational Bayesian methods allows the flexibility in modeling the data and are more numerically stable than usual recursive algorithms\cite{Naoki}. Subspace distribution is chosen to allow automatic relevance determination (ARD) and unlike the matrix or tensor completion works, the algorithm parameters such as rank, noise powers, and state noise powers need not be specified or tuned. \par 
% The proposed algorithm is tested on the air quality and traffic dataset. We compare the performance of the proposed algorithm with various state of the art algorithm. The result shows modelling of the evolution of the subspace and leads to improvement in performance and reduction in the number of sensor measurements. 

% Our contribution can be summarized as follows.
% \begin{itemize}
% 	\item We propose a novel Matrix completion framework that take into exploit the low rankness, state space model for temporal evolution and the subspace tracking over days. The subspace tracking algorithm used for the time series data that can capture the periodicity of the data over many days.. 
% 	\item We also showed that incorporating the previous subspace information can reduce the sample complexity thereby motivating VBFSI for extreme matrix completion.
% 	\item We present a Variational Bayesian Filtering with Subspace Information algorithm for spatio temporal data estimation where the rank is determined by Automatic relevance determination and is not tuned. 
% 	\item  We also propose a Robust version of Variational Bayesian Filtering with Subspace Information for estimating the data in the presence of outliers. 
	
% 	\item We perform comprehensive experiments on the real world spatio temporal datasets and synthetic dataset. 
	
% \end{itemize} 

\subsection{Related work }
\begin{itemize}
\item 	Big data matrices can be approximated as low-rank matrices \cite{udell2019big}. Matrix completion is used to exploit the low-rank structure in the data to impute the missing data  \cite{asif2016matrix,sparsebayesian}. Robust PCA is used for matrix completion in the presence of outliers by incorporating a sparse outlier matrix \cite{compare7,compare8}. The traditional matrix completion framework is not applicable for time series data imputation, as it does not take into account the ordering among the temporal embeddings \cite{compare1}. 
	\item Autoregressive model can model these temporal embeddings and in turn capture the temporal evolution in the time series data\cite{varst,compare1,compare6}. However, these models fail to capture the prior subspace information that can be exploited to capture periodicity in the time series data. \textbf{why do these not fit the EMC approach}
		\item Exploiting the 3-way pattern in the data using tensor completion-based frameworks can incorporate the periodic pattern in the data and, in turn, improve the imputation performance \cite{asif2016matrix,compare3,ten1}. These method works better than the traditional matrix completion framework. However, the temporal evolution and subspace evolution is not modeled in the traditional tensor completion frameworks. We propose to incorporate the periodicity in the matrix completion framework while modeling the temporal and subspace evolution over days.

\item Variational Bayesian approaches are proposed for matrix/tensor completion and robust principal component analysis by modeling the matrix/tensor as low rank \cite{sparsebayesian,var1,compare3,compare8,asif2016matrix}. A state-space model to capture the temporal evolution is also proposed in \cite{varst,compare6}. However, these approaches do not explicitly model the evolution of the subspace to capture the periodicity in the data.  
\item The proposed matrix and tensor completion methods are not evaluated for extreme data missing problem and missing data estimation problem in the presence of outliers. 


\end{itemize}

 The paper is organized as follows: Section 2 presents the Variational Bayesian Filtering with Subspace Information. Section 3 presents the Robust Variational Bayesian Filtering with Subspace Information. Results and findings for air quality estimation and traffic estimation are discussed in section 4 followed by conclusion in section 5.


\subsection{Notations}
Tensor is denoted by $\pmb{X}$, Matrix is denoted by $\X$, its transpose is denoted by $\X^T$. For a given day $d$ the matrix is denoted by $\X^d$, we represent it as $\X$ throughout the paper. For the rest of the days matrix is represented by $\X^k$ where $k=\{1,2 \dots d-1\}$. The $(i,j)$-th element of a matrix $\X$ is denoted by $X_{i,j}$, the $i$-th row by $\x_{i\dott}$ and the $i$-th column by $\x_{i}$.  The multivariate Gaussian probability density function (pdf) with mean vector $\mub$ and covariance matrix $\Sig$ evaluated at $\x \in \Rn^n$ is denoted by $\N(\x \mid \mub,\Sig)$.\par
  
  
  
  
  
 
  
 
       
%Monitoring air quality helps in assessing the level of pollution with air quality standards. Dense spatial air quality maps are not possible due to the expensive static sensors.The aim of the work is to generate dense spatio temporal map with moving sensor data. The number of sensors needed is just a fraction of the total number of nodes.We do not need static monitors at all the time and in all locations, one may move these monitor to sample at other locationsBuilding an anytime-anywhere map of air quality in a city is critical in mitigation of pollution and is an essential tool in fighting climate change. Hybrid of static and moving monitors can be further explored Recently We use the autoregressive model to capture the temporal evolution in the data. Subspace learned for a day is used to update the subspace for the next day. Based on the real-time variations, the subspace can be updated. We motivate the applicability of the proposed method on other spatio temporal maps like traffic measurements. Matrix completion has been for traffic data. However, online subspace learning over days are not yet Matrix completion based algorithms are not explored for 
%moving sensor paradigm can be an excellent candidate to obtain dense air quality maps with the actual number of sensors needed is just a fraction of the total number of nodes.



==> introduction_1.tex <==


\section{Introduction}
Copious amounts of sensors are deployed in major cities for sensing the spatio-temporal variation in various urban environment characteristics like air pollution, traffic speed, etc.  Hitherto, the most common way of sensing data across a city is to deploy many stationary sensors or monitors across the city. Ideally, these static monitors should have a dense spatial coverage to achieve a fine-grained local source apportionment. Deploying static sensors in such large numbers is not only expensive but also challenging to maintain, and as a result, most cities, especially in the developing world, have a sparse network of sensor monitors \cite{vardoulakis2005spatial}.  One way to improve the spatio-temporal data coverage is to use drive-by sensing or moving sensors that sample various parts of a region at different time instances.  \cite{intro_drive1,hasenfratz2015deriving}. Since one sensor can be used to sample many locations at different timestamps, the actual number of moving sensors needed is just a fraction of the total number of static sensors needed to get the same spatial coverage.
\par 
Data acquired from both static and moving sensors contains missing data due to sensor malfunction, irregularity in sensor measurements, etc.  Additionally, the drive-by sensing scheme uses relatively fewer sensors resulting in high data ``gaps" in both spatial and temporal dimensions \cite{intro_drive1}. This motivates the problem of extreme matrix completion, where the percentage of data sampled may be as low as $10\%$.  Hence, a natural question to ask is: how to fill the missing entries within a reasonable error range? In addition to the missing entries, sensor measurements can be contaminated with outliers emerging from the sensor malfunctioning, communication errors, or impulse noises. The occurrence of outliers in the measurements can further degrade the performance of data imputation. But, unlike the missing entries, the location and the value of outliers are not known, which makes the problem more challenging.  The other question to ask is: how to estimate the missing data while detecting the noisy outliers?  The answer to the above questions lies in exploiting the underlying structure available in the data. For instance, both the air pollution \cite{sampson2011pragmatic} and the traffic \cite{min2011real} data exhibit joint spatial and temporal correlation as well as temporal periodicity, thereby generating redundancy that can be potentially exploited by performing an intelligent spatio-temporal extrapolation.   \par

%Data collected from the sensors in transportation and environment, etc., have spatial variability and follows slowly varying pattern over time. One way of imputation is to exploit this spatiotemporal correlation in the data matrix, where one axis denotes the spatial variability, and the other axis indicates the temporal evolution.


We motivate the problem of spatio-temporal matrix completion as follows. For a given day $d$, the data is represented in the form of a matrix $\X \in \mathcal{R}^{n \times t}$  where  $n$ and  $t$ are the numbers of spatial locations and time slots respectively. Our goal is to estimate the missing entries in the matrix $\X$. We motivate a low-rank robust subspace filtering approach for online matrix imputation, specifically for the extreme scenario of very sparse spatio-temporal sensing. One way of imputation is to exploit the low-rank structure available in the data \cite{asif2016matrix}. However, enforcing only the low rank structure in the data does not take into account the temporal variation (generally slow variation) of the data in a given location \cite{compare1}.  We incorporate a state space model to capture the temporal evolution in the data. 
Moreover, exploiting reliable prior subspace information can reduce the sample complexity of matrix completion and improve the imputation performance \cite{prove1}. We update the subspace on  day $d$ using the prior subspace estimated of day $d-1$ to capture the periodicity in the data. Incorporating this prior subspace can improve the performance for an extreme case of sparsely sampled data. 

 We use the Variational Bayes approach to update the parameters in an iterative fashion. In our work, the subspace distribution is chosen to allow automatic relevance determination (ARD) and unlike the matrix or tensor completion methods, the algorithm parameters such as rank, noise powers, need not be specified or tuned. We compare the performance of the proposed algorithm with various state-of-the-art algorithms on many real world air quality and traffic datasets. The result shows modeling of the evolution of the subspace leads to improvement in performance even when a small percentage of random measurements are available for the purpose of imputation. A likely impact of our method is that cities with a low sensing budget can perform random drive-by sampling of the urban environment, and the suggested matrix completion framework can provide a reasonably accurate imputation leading to better decision making. \par 

Our main contribution can be summarized as follows.
\begin{itemize}
	\item  We propose Variational Bayesian Filtering with Subspace Information (VBFSI), a novel matrix completion framework that simultaneously models the low rank nature of the data, temporal evolution through a state space model, and periodicity through subspace tracking. 
	\item We experimentally showed that incorporating the prior subspace over days can improve imputation performance, especially for low data sampling.
	% <not clear> \item We also illustrate our subspace can reduce the sample complexity, thereby motivating VBFSI for extreme matrix completion.
	\item Critical parameter, like the rank of the model, is automatically tuned using the automatic relevance determination (ARD) approach. 
	\item  We also propose a Robust version of the VBFSI algorithm for imputing the data in the presence of outliers. 
	\item We conduct comprehensive experiments on real-world spatio-temporal datasets that show the efficacy of the proposed method over other state-of-the-art imputation methods. 
	
\end{itemize} 

\subsection{Related work }
Big data matrices can be approximated as low rank matrices \cite{udell2019big}. Matrix completion is used to exploit the  low rank structure in the data to impute the missing data  \cite{asif2016matrix,sparsebayesian}. Robust PCA is used for matrix completion in the presence of outliers by incorporating a sparse outlier matrix \cite{compare7,compare8}. The traditional matrix completion framework is not applicable for time series data imputation, as it does not take into account the ordering among the temporal embeddings \cite{compare1}. Autoregressive model can model these temporal embeddings and in turn capture the temporal evolution in the time series data\cite{varst,compare1,compare6}. However, these models fail to capture the prior subspace information that can be exploited to capture periodicity in the time series data. Exploiting the 3-way pattern in the data using tensor completion based frameworks can incorporate the periodic pattern in the data and, in turn improve the imputation performance \cite{asif2016matrix,compare3,ten1}. However, the temporal evolution and subspace evolution is not modeled in the traditional tensor completion frameworks. 

Variational Bayesian approaches are proposed for matrix/tensor completion and robust principal component analysis by modeling the matrix/tensor as low rank \cite{sparsebayesian,var1,compare3,compare8,asif2016matrix}. A state space model to capture the temporal evolution is also proposed in \cite{varst,compare6}. However, these approaches do not explicitly model the evolution of the subspace to capture the periodicity in the data.  



\subsection{Notations}
Tensor is denoted by $\pmb{X}$, Matrix is denoted by $\X$, its transpose is denoted by $\X^T$. For a given day $d$ the matrix is denoted by $\X^d$, we represent it as $\X$ throughout the paper. For the rest of the days matrix is represented by $\X^k$ where $k=\{1,2 \dots d-1\}$. The $(i,j)$-th element of a matrix $\X$ is denoted by $X_{i,j}$, the $i$-th row by $\x_{i\dott}$ and the $i$-th column by $\x_{i}$.  The multivariate Gaussian probability density function (pdf) with mean vector $\mub$ and covariance matrix $\Sig$ evaluated at $\x \in \Rn^n$ is denoted by $\N(\x \mid \mub,\Sig)$.\par

 The paper is organized as follows:  Section 2 presents the Variational Bayesian Filtering with subspace information. Results and findings for air quality estimation and traffic estimation are discussed in section 3 followed by conclusion in section 4.






==> introduction_2.tex <==


\section{Introduction}
Copious amounts of sensors are deployed in major cities for sensing the spatio-temporal variation in various urban environment characteristics like air pollution, traffic speed, etc.  Formerly, the most common way of sensing data across a city is to deploy many stationary sensors or monitors across the city. Ideally, these static monitors should have a dense spatial coverage to achieve a fine-grained local source apportionment. Deploying static sensors in such large numbers is not only expensive but also challenging to maintain, and as a result, most cities, especially in the developing world, have a sparse network of sensor monitors (\cite{vardoulakis2005spatial}).  One way to improve the spatio-temporal data coverage is to use drive-by sensing or moving sensors that sample various parts of a region at different time instances.  \cite{intro_drive1,hasenfratz2015deriving}. Since one sensor can be used to sample many locations at different timestamps, the actual number of moving sensors needed is just a fraction of the total number of static sensors needed to get the same spatial coverage.
\par 
Data acquired from both static and moving sensors contains missing data due to sensor malfunction, irregularity in sensor measurements, etc.  Additionally, the drive-by sensing scheme uses relatively fewer sensors resulting in high data ''gaps" in both spatial and temporal dimensions \cite{intro_drive1}. This motivates the problem of extreme matrix completion, where the percentage of data sampled may be as low as $10\%$.  Hence, a natural question to ask is: how to fill the missing entries within a reasonable error range? In addition to the missing entries, sensor measurements can be contaminated with outliers emerging from the sensor malfunctioning, communication errors, or impulse noises. The occurrence of outliers in the measurements can further degrade the performance of data imputation. But, unlike the missing entries, the location and the value of outliers are not known, which makes the problem more challenging.  The other question to ask is: how to estimate the missing data while detecting the noisy outliers?  The answer to the above questions lies in exploiting the underlying structure available in the data. For instance, both the air pollution \cite{sampson2011pragmatic} and the traffic \cite{min2011real} data exhibit joint spatial and temporal correlation as well as temporal periodicity, thereby generating redundancy that can be potentially exploited by performing an intelligent spatio-temporal extrapolation.   \par

%Data collected from the sensors in transportation and environment, etc., have spatial variability and follows slowly varying pattern over time. One way of imputation is to exploit this spatiotemporal correlation in the data matrix, where one axis denotes the spatial variability, and the other axis indicates the temporal evolution.


We motivate the problem of spatio-temporal matrix completion as follows. For a given day $d$, the data is represented in the form of a matrix $\X \in \mathcal{R}^{n \times t}$  where  $n$ and  $t$ are the numbers of spatial locations and time slots respectively. Our goal is to estimate the missing entries in the matrix $\X$. We motivate a low-rank robust subspace filtering approach for online matrix imputation, specifically for the extreme scenario of very sparse spatio-temporal sensing. One way of imputation is to exploit the low-rank structure available in the data \cite{asif2016matrix}. However, enforcing only the low rank structure in the data does not take into account the temporal variation (generally slow variation) of the data in a given location \cite{compare1}.  We incorporate a state space model to capture the temporal evolution in the data. Finally, to capture the periodicity over days, we update the subspace on day $d$ using the subspace estimated on day $d-1$. We formulate a optimisation problem to complete the matrix with above structures in place via a variational Bayes approach and solve in an iterative fashion. In our work, the subspace distribution is chosen to allow automatic relevance determination (ARD) and unlike the matrix or tensor completion methods, the algorithm parameters such as rank, noise powers, and state noise powers need not be specified or tuned. We compare the performance of the proposed algorithm with various state-of-the-art algorithms on many real world air quality and traffic datasets. The result shows modelling of the evolution of the subspace and leads to improvement in performance even in the case when only a small percentage of random measurements are available for the purpose of imputation \cite{prove1,prove2}. A likely impact of our method is that cities with low sensing budget can perform random drive-by sampling of urban environment and the suggested matrix completion framework can provide a reasonably accurate imputation leading to better decision making. \par 

Our contribution can be summarized as follows.
\begin{itemize}
	\item  The proposed VBFSI approach simultaneously models 1. the low rank nature of the data, 2. temporal evolution through a state space model, and 3. periodicity through subspace tracking and completes the data matrix in a Bayesian framework. Our approach specially works for an extreme case of sparsely sampled data. 
	% <not clear> \item We also illustrate our subspace  can reduce the sample complexity thereby motivating VBFSI for extreme matrix completion.
	\item Critical parameter like rank of the model is automatically tuned using the automatic relevance determination (ARD) approach. 
	\item  We also propose a Robust version of the VBFSI algorithm for imputing the data in the presence of outliers. 
	\item Comprehensive experiments on real world spatio-temporal datasets show that VBFSI outperforms the state-of-the-art imputation methods for most sampling frequencies. 
	
\end{itemize} 

\subsection{Related work }
Big data matrices can be approximated as low rank matrices \cite{udell2019big}. Matrix completion is used to exploit the  low rank structure in the data to impute the missing data  \cite{asif2016matrix,sparsebayesian}. Traditional matrix completion framework is no longer appropriate for time series applications, as it does not take into account the ordering among the temporal embeddings \cite{compare1}. Auto regressive model can capture these temporal embeddings and in turn capture the temporal evolution in the time series data\cite{varst,compare1,compare6}. However, these models fails to capture the prior subspace information which exists due to the periodicity in the time series data. Exploiting the 3-way pattern in the data using tensor completion based frameworks can further improve the imputation performance and model the periodic pattern in the data \cite{asif2016matrix,compare3,ten1}. These method works better than the traditional matrix completion framework. However, the temporal evolution and subspace evolution is not modeled in the traditional tensor completion frameworks. 

Variational Bayesian approaches are proposed for matrix/tensor completion and robust principal component analysis by modeling the matrix/tensor as low rank \cite{sparsebayesian,var1,compare3,compare8,asif2016matrix}. A state space model to capture the temporal evolution is also proposed in \cite{varst,compare6}. However, these approaches do not explicitly model the evolution of subspace to capture the periodicity in the data.  



\subsection{Notations}
Tensor is denoted by $\pmb{X}$, matrix is denoted by $\X$, its transpose is denoted by $\X^T$. The $(i,j)$-th element of a matrix $\X$ is denoted by $X_{i,j}$, the $i$-th column by $\x_{i}$, and the $i$-th row by $\x_{i\dott}$.  The multivariate Gaussian probability density function (pdf) with mean vector $\mub$ and covariance matrix $\Sig$ evaluated at $\x \in \Rn^n$ is denoted by $\N(\x \mid \mub,\Sig)$.







